Hawkeye: Reproducing GPU-Level Non-Determinism

We present Hawkeye, a system for analyzing and reproducing GPU-level arithmetic operations. Using our framework, anyone can re-execute on a CPU the exact matrix multiplication operations underlying a machine learning model training or inference workflow that was executed on an NVIDIA GPU, without any precision loss. This is in stark contrast to prior approaches to verifiable machine learning, which either introduce significant computation overhead to the original model owner, or suffer from non-robustness and quality degradation. The main technical contribution of Hawkeye is a systematic sequence of carefully crafted tests that study rounding direction, subnormal number handling, and order of (non-associative) accumulation during matrix multiplication on NVIDIA's Tensor Cores. We test and evaluate our framework on multiple NVIDIA GPU architectures ( Ampere, Hopper, and Lovelace) and precision types (FP16, BFP16, FP8). In all test cases, Hawkeye enables perfect reproduction of matrix multiplication on a CPU, paving the way for efficient and trustworthy third-party auditing of ML model training and inference. We provide source code for Hawkeye at https://github.com/badasherez/gpu-simulator.

==> open_science.tex <==
In accordance with the USENIX Security 2026 open‐science policy, we have made all artifacts required to reproduce and evaluate our results available at submission time.  Acceptance of this paper is conditional on these artifacts remaining publicly accessible (anonymized) throughout review.

\medskip\noindent\textbf{Source Code}:  
\begin{itemize}
      \item Repository: \url{https://github.com/anon4783/gpu-simulator.git}  
      \item Contents: Python scripts to reproduce the results of our experiments and GPU bit-exact emulators for Ampere and Hopper.
\end{itemize}

All links are available and do not require credentials. We have verified that the scripts run successfully and produce the correct end-to-end result using NVIDIA Tensor Cores on both Ampere and Hopper GPUs.

\paragraph{Licensing \& Restrictions}  
All code and data are released under the MIT License.  No artifacts are withheld for licensing or security reasons.

\paragraph{Artifact Evaluation}  
Upon conditional acceptance, we will provide non‐anonymized URLs and register our repository with the USENIX Security Artifact Evaluation service for optional functionality and reproducibility checks.  
